This is the Way: Differential Bayesian Filtering for Agile Trajectory Synthesis

One of the main challenges in autonomous racing is to design algorithms for motion planning at high speed, and across complex racing courses. End-to-end trajectory synthesis has been previously proposed where the trajectory for the ego vehicle is computed based on camera images from the racecar. This is done in a supervised learning setting using behavioral cloning techniques. In this paper, we address the limitations of behavioral cloning methods for trajectory synthesis by introducing Differential Bayesian Filtering (DBF), which uses probabilistic B\'ezier curves as a basis for inferring optimal autonomous racing trajectories based on Bayesian inference. We introduce a trajectory sampling mechanism and combine it with a filtering process which is able to push the car to its physical driving limits. The performance of DBF is evaluated on the DeepRacing Formula One simulation environment and compared with several other trajectory synthesis approaches as well as human driving performance. DBF achieves the fastest lap time, and the fastest speed, by pushing the racecar closer to its limits of control while always remaining inside track bounds.

==> sections/differential_bayesian_filtering/dbf_algorithm.tex <==
% \vspace{-3mm}
\begin{algorithm}

    \setlength{\textfloatsep}{0pt}
    \begin{algorithmic}
        \Procedure{DBF}{()} \\
            \State $p(\theta)$ \gets \mathcal{N}(AdmiralNet(), \begin{bmatrix} 1.0 & 0 \\ 0 &   1.0\end{bmatrix})\\
            \While{$\neg$ terminate()}
                    \State\ \ \ \ //Draw N samples from prior (each sample is\\\ \ \ \ //control points for a B\`ezier Curve) \\
                    \State\ \ \ \ $\{\theta_1, \theta_2, ... \theta_N\}$ \gets sample($p(\theta)\}$) \\
               %g \For{$i \in \{\}$}
                    \State\ \ \ \ //Compute derivatives for each sampled curve \\
                    \State\ \ \ \ $\mathcal{T}_{\theta_i}$ \gets \text{B\`ezier Curve defined by }$\theta_i$ \\
                    \State\ \ \ \ $\dot{\mathcal{T}_{\theta_i}}$ \gets  \text{Velocity of  }\mathcal{T}_{\theta_i} \\
                    \State\ \ \ \ $\ddot{\mathcal{T}_{\theta_i}}$ \gets  \text{Acceleration of  }\mathcal{T}_{\theta_i}  \\
                    \State\ \ \ \ //Compute weighting factors based on equation \ref{eqn:gamma}\\
                    \State\ \ \ \ $\gamma_i$ \gets \gamma(\mathcal{T}_{\theta_i}, \dot{\mathcal{T}_{\theta_i}}, \ddot{\mathcal{T}_{\theta_i}})  \\
              %  \EndFor
                
                    \State\ \ \ \ //Posterior is weighted sum of sampled curves\\
                          \ \ \ \ $\bar{\theta} = \sum_{i=1}^N\gamma_i*\theta_i$\\
                
               % \State //Resample based on probabilities $\gamma_i$\\
            %    \State $\{\theta_1, \theta_2, ... \theta_N\}$ \gets sample($\{\theta_i, \gamma_i\}$) \\
                
                    \State\ \ \ \ $p(\theta)$ \gets \mathcal{N}(\bar{\theta}, \begin{bmatrix} 1.0 & 0 \\ 0 &   1.0\end{bmatrix})
                
            \EndWhile
            \State \textbf{return} $p(\theta)$
        \EndProcedure
    \caption{Differential Bayesian Filtering}
    \end{algorithmic}
%\caption{The high-level loop of our approach.  AdmiralNet() is a call to our neural network and the point estimate it returns is the mean of our prior.}
    \label{alg:dbf}
% \vspace{-3mm}
\end{algorithm}
